A Category Theoretic View of Contextual Types: from Simple Types to Dependent Types

We describe the categorical semantics for a simply typed variant and a simplified dependently typed variant of Cocon, a contextual modal type theory where the box modality mediates between the weak function space that is used to represent higher-order abstract syntax (HOAS) trees and the strong function space that describes (recursive) computations about them. What makes Cocon different from standard type theories is the presence of first-class contexts and contextual objects to describe syntax trees that are closed with respect to a given context of assumptions. Following M. Hofmann's work, we use a presheaf model to characterise HOAS trees. Surprisingly, this model already provides the necessary structure to also model Cocon. In particular, we can capture the contextual objects of Cocon using a comonad $\flat$ that restricts presheaves to their closed elements. This gives a simple semantic characterisation of the invariants of contextual types (e.g. substitution invariance) and identifies Cocon as a type-theoretic syntax of presheaf models. We further extend this characterisation to dependent types using categories with families and show that we can model a fragment of Cocon without recursor in the Fitch-style dependent modal type theory presented by Birkedal et. al..

==> figures/semmodel.tex <==
\begin{figure}[hbt]
  \centering\small
  \[
    \begin{array}{c}
      \multicoltext{Basic structure}\\
      \Istype{\Ctx}
      \qquad
      \Istype[\Gamma, \Phi : \Ctx]{El(\Phi)}
      \qquad      
      \Istype[\Gamma, \Phi : \Ctx]{Ty(\Phi)}
      \qquad
      \typing{\top}{\Ctx}
      \qquad
      \typing{\top}{El(\top)}

      \\[0.5em]
      
      \typing{.}{(\Phi : \Ctx) \to (A : Ty(\Phi)) \to \Ctx}
      \qquad
      \typing[\Gamma, \Phi : \Ctx]{!}{El(\Phi) \to El(\top)}
      \qquad
      \typing[\Gamma, \Phi : \Ctx, A : Ty(\Phi)]{p}{El(\Phi.A) \to El(\Phi)}

      \\[0.5em]
      
      \typing[\Gamma, \Phi : \Ctx, \Psi : \Ctx, \sigma : El(\Phi) \to El(\Psi)]
      {-\{\sigma\}}{Ty(\Psi) \to Ty(\Phi)}

      \\[0.5em]
      
      \typing[\Gamma,\Phi : \Ctx, \Psi : \Ctx, A : Ty(\Psi), \sigma : El(\Phi) \to
      El(\Psi)] {q(\sigma, A)}{El(\Phi.A\{\sigma\}) \to El(\Psi.A)}

      \\[0.5em]
      
      \Istype[\Gamma, \Phi : \Ctx, A : Ty(\Phi)]
      {Tm(\Phi, A) \equiv \Sigma (El(\Phi) \to El(\Phi.A)) (\lambda M . p \circ M = 1_\Phi)}

      \\[0.5em]
      \typing[\Gamma, \Phi,\Psi : \Ctx, A : Ty(\Psi), \sigma : El(\Phi) \to El(\Psi)]
      {-\{\sigma\}}{Tm(\Psi, A) \to Tm(\Phi, A\{\sigma\})}

      \\[0.5em]
      \typing[\Gamma, \Phi: \Ctx, u : El(\Phi), A : Ty(\Phi), M : Tm(\Phi, A)]
      {M(u)}{El(\Phi.A)}

      \\[0.5em]

      \typing[\Gamma, \Phi : \Ctx, A : Ty(\Phi)]{v}{Tm(\Phi.A, A\{p\})}
      
      \\[0.5em]

      \typing[\Gamma, \Psi, \Phi : \Ctx, \sigma : El(\Phi) \to El(\Psi), M : Tm(\Psi,
      A\{\sigma\})]{\ctxext{\sigma, M}}{El(\Psi) \to El(\Phi.A)}

      \\[1em]
      \multicoltext{$\Pi$ types}\\
      \inferrule*
      {\typing[\Gamma, \Phi : \Ctx]{A}{Ty(\Phi)} \\
      \typing[\Gamma, \Phi : \Ctx]{B}{Ty(\Phi.A)} }
      {\typing[\Gamma, \Phi : \Ctx]{\Pi(A, B)}{Ty(\Phi)}}
      \qquad
      \inferrule*
      {\typing[\Gamma, \Phi : \Ctx]{M}{Tm(\Phi.A, B)}}
      {\typing[\Gamma, \Phi : \Ctx]{\Lambda(M)}{Tm(\Phi, \Pi(A, B))}}

      \\[0.5em]
      
      \inferrule*
      {\typing[\Gamma, \Phi : \Ctx]{M}{Tm(\Phi, \Pi(A, B))} \\
      \typing[\Gamma, \Phi : \Ctx]{N}{Tm(\Phi, A)}}
      {\typing[\Gamma, \Phi : \Ctx]{App(M, N)}{Tm(\Phi, B\{N\})}}

      \\[1em]
      \multicoltext{Model for the object language in LF}\\
      \typing{ty}{Ty(\top)}
      \qquad
      \typing{trm}{Ty(\top.ty)}
      \qquad
      \typing[\Gamma, \Phi:\Ctx]{ty\{!\}}{Ty(\Phi)}
      \qquad
      ty' \equiv ty\{!\} : Ty(\Phi)

      \\[0.5em]
      \inferrule*
      {\sigma \equiv \ctxext{!, a} : El(\Phi) \to El(\top.ty)}
      {\typing[\Gamma, \Phi : \Ctx, a : Tm(\Phi, ty')]{trm[a] \equiv trm\{\sigma\}}{Ty(\Phi)}}

      \\[0.5em]
      \typing[\Gamma, \Phi : \Ctx]{o}{Tm(\Phi, ty')}
      \qquad
      \typing[\Gamma, \Phi : \Ctx] {arr} {Tm(\Phi, ty') \to Tm(\Phi, ty') \to
      Tm(\Phi, ty')}

      \\
      \typing[\Gamma, \Phi : \Ctx]
      {lam}
      {(a, b : Tm(\Phi, ty')) \to
      Tm(\Phi.trm[a], trm[b\{p\}]) \to
      Tm(u, trm[arr(a, b)])}

      \\
      \typing[\Gamma, \Phi : \Ctx]
      {app}
      {(a, b : Tm(\Phi, ty')) \to
      Tm(\Phi, trm[arr(a, b)]) \to
      Tm(\Phi, trm[a]) \to Tm(u, trm[b])}

    \end{array}
  \]
  \caption{Semantic Model}\label{fig:semmodel}
\end{figure}

==> makefile <==
.PHONY: all clean

TARGETS:=main.pdf response.pdf response1.pdf template.pdf
TOREMOVE:=$(filter-out *.pdf,$(shell cat .gitignore))
TEXFILES:=$(subst ./,,$(shell find . -name '*.tex'))

all:main.pdf response.pdf

${TARGETS}: %.pdf: %.tex $(filter-out $(subst .pdf,.tex,${TARGETS}),${TEXFILES})
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)
	bibtex $(@:.pdf=)
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)

temp.pdf: temp.tex
	bibtex $(@:.pdf=) || true
	pdflatex -shell-escape -halt-on-error $(@:.pdf=)

FINDCMDPRE:=${foreach x, ${TOREMOVE}, -o -name '$x'}
FINDCMD:=${wordlist 2,${words ${FINDCMDPRE}},${FINDCMDPRE}}

clean:
	find . \( ${FINDCMD} \) -exec rm -rf {} +
	find . -name '_minted*' -exec rm -r {} +
	rm main.pdf

